IterCQR: Iterative Conversational Query Reformulation with Retrieval Guidance

Conversational search aims to retrieve passages containing essential information to answer queries in a multi-turn conversation. In conversational search, reformulating context-dependent conversational queries into stand-alone forms is imperative to effectively utilize off-the-shelf retrievers. Previous methodologies for conversational query reformulation frequently depend on human-annotated rewrites. However, these manually crafted queries often result in sub-optimal retrieval performance and require high collection costs. To address these challenges, we propose Iterative Conversational Query Reformulation (IterCQR), a methodology that conducts query reformulation without relying on human rewrites. IterCQR iteratively trains the conversational query reformulation (CQR) model by directly leveraging information retrieval (IR) signals as a reward. Our IterCQR training guides the CQR model such that generated queries contain necessary information from the previous dialogue context. Our proposed method shows state-of-the-art performance on two widely-used datasets, demonstrating its effectiveness on both sparse and dense retrievers. Moreover, IterCQR exhibits superior performance in challenging settings such as generalization on unseen datasets and low-resource scenarios.

==> Table/CaST.tex <==
\begin{table}[th]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{\extracolsep{5pt}}l|c|cccc@{}}
\toprule[1.5pt]

\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Human}\\\textbf{Rewrite}\end{tabular}}& \multicolumn{2}{c}{\textbf{CAsT-19}}                      & \multicolumn{2}{c}{\textbf{CAsT-20}} \\   
\cline{3-4} \cline{5-6}
\multicolumn{1}{c|}{}                 &      & \multicolumn{1}{c}{MRR} & \multicolumn{1}{c}{NDCG@3} & \multicolumn{1}{c}{MRR} & \multicolumn{1}{c}{NDCG@3} \\
\hline
\textbf{Human-Rewrite} & O& 0.740 & 0.461 & 0.591 & 0.422\\ 
\hline
\textbf{Transformer++} &O& 0.696 &\textbf{0.441} & 0.296 & 0.185 \\
\textbf{Query Rewriter}&O & 0.665 & 0.409 & 0.375 & 0.255 \\
\textbf{CQE-Sparse} &O& 0.671 & 0.399 & 0.423 & 0.271 \\
\textbf{QuReTeC}&O & 0.689 & 0.430 & 0.430 & 0.287 \\
\textbf{T5QR} &O& 0.701 & 0.417 & 0.423 & 0.299 \\
\textbf{ConvGQR} &O& \textbf{0.708} & 0.434 & \textbf{0.465} & \textbf{0.331} \\
\hline
\textbf{IterQR} &X& 0.655 & 0.400 & 0.378 & 0.180 \\ 
\textbf{IterQR\small{+expansion}} &X& 0.693 & 0.428 & 0.402 & 0.190 \\ 
\bottomrule[1.5pt]
\end{tabular}%
}
\caption{CAsT-19 \& CAsT-20 Zero-shot Results}
\label{table:cast}
\end{table}



==> Table/qrecc_example.tex <==
\begin{table*}
\centering\resizebox{\textwidth}{!}{
\begin{tabular}{>{\hspace{0pt}}m{0.25\linewidth}>{\hspace{0pt}}m{0.25\linewidth}>{\hspace{0pt}}m{0.5\linewidth}} 
\toprule [1.5pt]
\textbf{Original Query} & \textbf{Human Rewrite} & \textbf{IterCQR Query} \\ 
\hline
Was there any controversy with \textcolor{red}{ the agency} & Was there any controversy with \textcolor{red}{nsw} & Was there any controversy surrounding the agency \textcolor[rgb]{0,0.388,0}{WorkCover }\textcolor{red}{NSW}'s \textcolor[rgb]{0,0.388,0}{regulations }to promote productive, \textcolor[rgb]{0,0.388,0}{healthy and safe workplaces} for workers in \textcolor[rgb]{0,0.388,0}{New South Wales.} \\
\textbf{Gold Answer} & \multicolumn{2}{>{\hspace{0pt}}m{0.885\linewidth}}{In December 2005, the Independent Commission Against Corruption found that 23 NSW WorkCover employees had issued false certificates of competency.} \\
\textbf{Gold Passage} & \multicolumn{2}{>{\hspace{0pt}}m{0.885\linewidth}}{Dangerous Goods (Gas Installations) Regulation 1998 (\textcolor{red}{NSW}) Dangerous Goods (Road and Rail Transport) Regulation 2009 (NSW) Explosives Regulation 2005 (\textcolor{red}{NSW}) Occupational~\textcolor[rgb]{0,0.388,0}{\textbf{\textbf{Health}}}~and\textbf{\textbf{~\textcolor[rgb]{0,0.388,0}{Safety}~\textcolor[rgb]{0,0.388,0}{Regulation~}}}2001 (\textcolor{red}{NSW}) Sporting Injuries Insurance Regulation 2009 (\textcolor{red}{NSW}) Workers Compensation (Bush Fire, Emergency and Rescue Services) Regulation 2007 (\textcolor{red}{NSW}) Workers' Compensation (Dust Diseases) Regulation 2008 (\textcolor{red}{NSW}) Workers Compensation Regulation 2010 (\textcolor{red}{NSW}) Standards [ edit ] Australian standards outline safety requirements and give guidance to people working in certain areas or people that use certain equipment. When incorporated into legislation these standards become legally binding. Under~\textcolor{red}{NSW}~law, a variety of systems, equipment, products and materials must meet Australian Standards. The establishment of standards ensures that particular requirements are met. The requirements that are outlined are quality, performance, construction design, endurance time specificity, systems or processes and certain hazards and controls. Controversy [ edit ]\textbf{\textbf{~\uline{In December 2005, the Independent Commission Against Corruption found that 23~\textcolor[rgb]{0,0.388,0}{WorkCover}~employees had issued false certificates of competency}}}, which ICAC states significantly undermined~\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{workplace}~}}safety on building sites. [18] ICAC further states that systemic corruption risks were exposed by the incident: [The ICAC] identified a number of deficiencies such as sharing of logon details and passwords, lack of supervision and controls in approving and printing certificates of competency, and lack of reconciliation between certificates issued and applicant fees. [18] In 2002, a\textbf{\textbf{~\textcolor[rgb]{0,0.388,0}{New South Wales}}}~parliamentary committee criticized the~\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{WorkCover}}}~Authority. [19]} \\ 
\hdashline
When was \textcolor{red}{the agency} formed & when was \textcolor{red}{nsw} formed & When was the \textcolor{red}{NSW} WorkCover agency formed to \textcolor[rgb]{0,0.388,0}{promote productive, healthy and safe workplaces for workers in New South Wales.} \\
\textbf{Gold Passage} & \multicolumn{2}{>{\hspace{0pt}}m{0.885\linewidth}}{The WorkCover Authority of New South Wales was a New South Wales Government agency established in 1989.} \\
\textbf{Gold Passage} & \multicolumn{2}{>{\hspace{0pt}}m{0.885\linewidth}}{'\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{WorkCover}}}~Authority of~\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{New South Wales}}}~- Wikipedia CentralNotice~\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{WorkCover}}}~Authority of~\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{New South Wales}}}~From Wikipedia, the free encyclopedia Jump to navigation Jump to search Authority of~\textcolor[rgb]{0,0.388,0}{\textbf{\textbf{New South Wales}}}~Statutory authority overview Formed 1989 Dissolved 2015 Jurisdiction~\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{New South Wales}}}~Parent Statutory authority Department of Finance and Services Key documents Safety, Return to Work and Support Board Act, 2012 (NSW) Work Health and Safety Act, 2011 (NSW) Website~\textcolor[rgb]{0,0.388,0}{\textbf{\textbf{workcover}}}~.nsw .gov .au The\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{~WorkCover}}}~Authority of~\textcolor[rgb]{0,0.388,0}{\textbf{\textbf{New South Wales}}}~or~\textcolor[rgb]{0,0.388,0}{\textbf{\textbf{WorkCover}}}~NSW is a~\textcolor[rgb]{0,0.388,0}{\textbf{\textbf{New South Wales~}}}Government agency established in 1989. The agency creates regulations to~\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{promote productive, healthy and safe~workplaces for workers}~}}and employers in~\textcolor[rgb]{0,0.388,0}{\textbf{\textbf{New South Wales}}.}~[1] The agency formed part of the Safety, Return to Work and Support Division established pursuant to the Safety, Return to Work and Support Board Act, 2012 (NSW). On 1 September 2015,~\textbf{\textbf{\textcolor[rgb]{0,0.388,0}{WorkCover~}}}NSW was replaced by three new entities – Insurance and Care NSW (icare), [2] the State Insurance Regulatory Authority (SIRA), [3] and SafeWork NSW, [4] the new work health and safety regulator. The changes were part of reforms to improve the workers compensation system for employers and injured workers. The information below pertains to the former~\textcolor[rgb]{0,0.388,0}{\textbf{\textbf{WorkCover}}}~NSW.~\textcolor[rgb]{0,0.388,0}{\textbf{\textbf{WorkCover}}}~NSW no longer exists, however its functions have been split between the aforementioned newly created agencies.} \\
\bottomrule [1.5pt]
\end{tabular}}
\caption{Reformulated Queries by IterCQR on QReCC dataset.}
\label{table:qrecc_example}
\end{table*}

==> Table/zero_shot.tex <==
% \begin{table*}[th]
% \centering\resizebox{\textwidth}{!}{
% \begin{tabular}{@{\extracolsep{8pt}}ccc|cccccccc@{}}
% \toprule[1.5pt]
% \multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{Test}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{TopiOCQA test}} & \multicolumn{4}{c}{\textbf{QReCC test}} \\ 
% \cline{4-7} \cline{8-11}
%  &  &  & \textbf{MRR} & \textbf{NDCG@3} & \textbf{R@10} & \textbf{R@100} & \textbf{MRR} & \textbf{NDCG@3} & \textbf{R@10} & \textbf{R@100} \\ 
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Dense}\\(ANCE)\end{tabular}} & \multirow{2}{*}{\textbf{ID}} & \textbf{CONQRR} & - & - & - & - & 0.418 & - & \textbf{65.1} & \textbf{84.7} \\
%  &  & \textbf{ConvGQR} & \textbf{0.256} & \textbf{0.243} & \textbf{41.8} & \textbf{58.8} & \textbf{0.420} & \textbf{0.391} & 63.5 & 81.8 \\ 
% \cline{2-11}
%  & \textbf{OOD} & \textbf{IterCQR} & 0.178 & 0.163 & 29.6 & 48.1 & 0.401 & 0.374 & 61.8 & 80.1 \\ 
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Sparse}\\(BM25)\end{tabular}} & \multirow{2}{*}{\textbf{ID}} & \textbf{CONQRR} & - & - & - & - & 0.383 & - & 60.1 & \textbf{88.9} \\
%  &  & \textbf{ConvGQR} & 0.124 & 0.107 & \textbf{23.8} & \textbf{45.6} & 0.441 & 0.410 & \textbf{64.4} & 88.0 \\ 
% \cline{2-11}
%  & \textbf{OOD} & \textbf{\textbf{IterCQR}} & \textbf{0.137} & \textbf{0.122} & 23.4 & 45.1 & \textbf{0.449} & \textbf{0.424} & 62.5 & 83.8\\
% \bottomrule[1.5pt]
% \end{tabular}}
%   \caption{ IterCQR performance in domain-shift scenarios. CONQRR and ConvGQR are reported by in-domain setting while IterCQR is evaluated in OOD setting. For the TopiOCQA test case, ConvGQR was trained on TopiOCQA while IterCQR was trained on QreCC. For the QRecc test case, ConvGQR and CONQRR were trained on QreCC while IterCQR was trained on TopiOCQA.  }
%   \label{table:zero_shot}
% \end{table*}


\begin{table*}[th]
\centering\resizebox{\textwidth}{!}{
\begin{tabular}{@{\extracolsep{8pt}}ccc|cccccccc@{}}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{Test}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{TopiOCQA Test}} & \multicolumn{4}{c}{\textbf{QReCC Test}} \\ 
\cline{4-7} \cline{8-11}
 &  &  & \textbf{MRR} & \textbf{NDCG@3} & \textbf{R@10} & \textbf{R@100} & \textbf{MRR} & \textbf{NDCG@3} & \textbf{R@10} & \textbf{R@100} \\ 
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Dense}\\(ANCE)\end{tabular}} & \multirow{2}{*}{\textbf{ID}} & \textbf{\textsc{Con}QRR} & - & - & - & - & 0.418 & - & {65.1} & {84.7} \\
 &  & \textbf{ConvGQR} & {0.256} & 0.243 & {41.8} & {58.8} & {0.420} & {0.391} & 63.5 & 81.8 \\ 
\cline{2-11}
 & \textbf{OOD} & \textbf{IterCQR} & 0.178 & 0.163 & 29.6 & 48.1 & 0.401 & 0.374 & 61.8 & 80.1 \\ 
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Sparse}\\(BM25)\end{tabular}} & \multirow{2}{*}{\textbf{ID}} & \textbf{\textsc{Con}QRR} & - & - & - & - & 0.383 & - & 60.1 & {88.9} \\
 &  & \textbf{ConvGQR} & 0.124 & 0.107 & {23.8} & {45.6} & 0.441 & 0.410 & {64.4} & 88.0 \\ 
\cline{2-11}
 & \textbf{OOD} & \textbf{\textbf{IterCQR}} & {0.137} & {0.122} & 23.4 & 45.1 & {0.449} & {0.424} & 62.5 & 83.8\\
\bottomrule[1.5pt]
\end{tabular}}
  \caption{ IterCQR performance in domain-shift scenarios. \textsc{Con}QRR and ConvGQR are reported by in-domain setting while IterCQR is evaluated in OOD setting. For the TopiOCQA test case, ConvGQR was trained on TopiOCQA while IterCQR was trained on QReCC. For the QReCC test case, ConvGQR and \textsc{Con}QRR were trained on QReCC while IterCQR was trained on TopiOCQA.  }
  \label{table:zero_shot}
\vspace{-3mm}
\end{table*}




==> Table/zero_shot3.tex <==

\begin{table*}[t]
\small\centering\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.2}
% \begin{tabular}{@{\extracolsep{8pt}}cc|cccc | cccc@{}}
\begin{tabular}{cc|cc|cc|cc|cc}
\toprule [1.5pt]
\multirow{3}{*}{\textbf{Test}} &
  \multirow{3}{*}{\textbf{Method}} &
  \multicolumn{4}{c|}{\textbf{TopiOCQA Test}} &
  \multicolumn{4}{c}{\textbf{QReCC Test}} \\ \cline{3-10} 
 &
   &
  \multicolumn{2}{c}{\textbf{Dense}} &
  \multicolumn{2}{c|}{\textbf{Sparse}} &
  \multicolumn{2}{c}{\textbf{Dense}} &
  \multicolumn{2}{c}{\textbf{Sparse}} \\
 &
   &
  \multicolumn{1}{c}{\textbf{MRR}} &
  \multicolumn{1}{c}{\textbf{NDCG@3}} &
  \multicolumn{1}{c}{\textbf{MRR}} &
  \multicolumn{1}{c|}{\textbf{NDCG@3}} &
  \multicolumn{1}{c}{\textbf{MRR}} &
  \multicolumn{1}{c}{\textbf{NDCG@3}} &
  \multicolumn{1}{c}{\textbf{MRR}} &
  \multicolumn{1}{c}{\textbf{NDCG@3}} \\ \hline
\multirow{2}{*}{\textbf{ID}} &
  \textbf{\textsc{Con}QRR}  & - & - & - & - & 0.418 & - & 0.383 & - \\
 &
  \textbf{ConvGQR} & 0.256 & 0.243 & 0.124 & 0.107 & 0.420 & 0.391 & 0.441 & 0.410 \\ 
\textbf{OOD} &
  \textbf{IterCQR} & 0.178 & 0.163 & 0.137 & 0.122 & 0.401 & 0.374 & 0.449 & 0.424 \\
\bottomrule[1.5pt]
\end{tabular}
}
    \caption{ IterCQR performance in unseen datasets. \textsc{Con}QRR and ConvGQR are reported for an in-domain setting while IterCQR is evaluated in OOD setting. For the TopiOCQA test case, ConvGQR was trained on TopiOCQA while IterCQR was trained on QReCC. For the QReCC test case, ConvGQR and \textsc{Con}QRR were trained on QReCC while IterCQR was trained on TopiOCQA.  }
    \label{table:zero_shot3}
\end{table*} 

